Hardness of Approximation of Euclidean $k$-Median

The Euclidean $k$-median problem is defined in the following manner: given a set $\mathcal{X}$ of $n$ points in $\mathbb{R}^{d}$, and an integer $k$, find a set $C \subset \mathbb{R}^{d}$ of $k$ points (called centers) such that the cost function $\Phi(C,\mathcal{X}) \equiv \sum_{x \in \mathcal{X}} \min_{c \in C} \|x-c\|_{2}$ is minimized. The Euclidean $k$-means problem is defined similarly by replacing the distance with squared distance in the cost function. Various hardness of approximation results are known for the Euclidean $k$-means problem. However, no hardness of approximation results were known for the Euclidean $k$-median problem. In this work, assuming the unique games conjecture (UGC), we provide the first hardness of approximation result for the Euclidean $k$-median problem. Furthermore, we study the hardness of approximation for the Euclidean $k$-means/$k$-median problems in the bi-criteria setting where an algorithm is allowed to choose more than $k$ centers. That is, bi-criteria approximation algorithms are allowed to output $\beta k$ centers (for constant $\beta>1$) and the approximation ratio is computed with respect to the optimal $k$-means/$k$-median cost. In this setting, we show the first hardness of approximation result for the Euclidean $k$-median problem for any $\beta < 1.015$, assuming UGC. We also show a similar bi-criteria hardness of approximation result for the Euclidean $k$-means problem with a stronger bound of $\beta < 1.28$, again assuming UGC.

==> bicriteria.tex <==
\section{Bicriteria Approximation for Discrete $k$-means}

We use a bicriteria hardness result for hypergraph vertex coverage to prove the bicriteria hardness result for discrete $k$-means and discrete $k$-median problems. We start by defining some problems and state the bicriteria hardness result for hypergraph vertex coverage problem that will be used crucially to prove the bicriteria hardness result for discrete $k$-means and discrete $k$ median problems.

\begin{definition}[$d$-hypergraph cover] Given a $d$-uniform hypergraph with $M$ vertices and $N$ hyperedges, the objective is to find a minimum cardinality subset of vertices that covers all hyperedges. \end{definition}

\begin{definition}[$t$-$d$-hypergraph cover] In $t$-$d$-hypergraph cover or hypergraph coverage problem, we are given a $d$-uniform hypergraph with $M$ vertices and $N$ hyperedges, and the objective is to find a subset of vertices of size $t$ that covers the maximum number of hyperedges. \end{definition}

\begin{definition}[Discrete $k$-means] In the Euclidean discrete $k$-means problem, we are given a set $X\subseteq \R^M$ of points to be clustered and a set $\mathcal{C}\subseteq \R^M$ of candidate centers and an integer $k$. The objective is to choose a set $C\subseteq \mathcal{C}$ of $k$ centers such that the $k$-means cost is minimized. \end{definition}


Next, we state the bicriteria hardness result for the hypergraph coverage problem from Chuzhoy \etal~\cite{CGHKKKN2005}.
\begin{theorem}{\cite{CGHKKKN2005}} \label{thm:inapproxChuzhoy} Let $n,d,\beta$ be large positive integers. Given a $d$-uniform hypergraph $\mathcal{H}=(V,F)$ with $M=n^{O({\log d})} {2^d}^{\beta}$ vertices and $N={2^d}^{\beta} M$ hyperedges, it is $\mathsf{NP}$-hard to distinguish, whether all hyperedges can be covered using some subset of $\frac{3M}{d}$ vertices or no subset of vertices of size at most $(1-\frac{1}{2d})M$ covers more than a $(1-\frac{1}{d{{2^d}^{\beta}}})N$ hyperedges. \end{theorem}


Let $t=\frac{3M}{d}$. We set $d$ such that there exists $\gamma>0$ for which $(1-\frac{1}{2d})M\geq (1+\gamma)\frac{3M}{d}$. Next, we show a reduction from the hypergraph coverage to the discrete $k$-means or discrete $k$-median problems. Similar constructions have been used in the work of Cohen-Addad and Kartik \cite{hardness:addad19} to prove the hardness results for discrete $k$-means and $k$-median problems. 

We construct a bipartite graph $G(L\cup R, E)$, where the set $L$ of vertices corresponds to the set of $M$ vertices in the $d$-uniform hypergraph $\mathcal{H}$, the set of vertices in $R$ corresponds to the set of $N$ hyperedges in $\mathcal{H}$. For any vertex $u\in V$ in $\mathcal{H}$, we have a vertex $l_u\in L$ and for any edge $f\in F$ in $\mathcal{H}$, we have a vertex $r_f\in R$. For any $l_u\in L$ and $r_f\in R$, we have an edge $(l_u,r_f) \in E$, if $u\subseteq f$. The instance for the discrete $k$-means problem is constructed using an embedding of the vertices and edges of this bipartite graph. We have vectors $e_1,\ldots,e_M\in \{0,1\}^M$ as embedding of $M$ vertices in $L$, where $e_i$ stands for the $i$th indicator vector in $\R^M$ with $i$th entry $1$ and the rest of the entries $0$. These vectors (points) form the set $C$ of centers for the discrete $k$-means problem. For each of the $N$ vertices in $R$ that corresponds to a hyperedge $(u_1,u_2,\ldots,u_d)\in F$, we have a point $(e_{u_1}+e_{u_2}+\ldots+e_{u_d})\in \R^M$. These points form the set $X$ of points to be clustered using discrete $k$-means. Let $k=\frac{3M}{d}$. The discrete $k$-means instance is given as $(X,C,k)$.

For any candidate center $c\in C$ corresponding to a vertex $l_u$ in $L$ and any point $x\in X$ corresponding to a vertex $r_f\in R$, we have $d(x,c)^2=(d-1)$ if $u\subseteq f$, $d(x,c)^2=(d+1)$ otherwise. When all hyperedges are covered using $k=\frac{3M}{d}$ vertices, any point $x\in X$ is at squared Euclidean distance $(d-1)$ from some set of $k$ centers in $C$. For those set of $k$ centers, the $k$-means cost is $(d-1)N$. And when for any set of $(1-\frac{1}{2d})M$ vertices covers at most $(1-\frac{1}{d{{2^d}^{\beta}}})N$ hyperedges, then the $k$-means cost is at least $(d-1) (1-\frac{1}{d{{2^d}^{\beta}}}) N + (d+1) \frac{1}{d{{2^d}^{\beta}}} N=(d-1)N\left[1+\frac{2}{d(d-1){{2^d}^{\beta}}}\right]$. Since, following Theorem \ref{thm:inapproxChuzhoy}, it is $\mathsf{NP}$-hard to distinguish between the above two cases, the inapproximability result for the discrete $k$-means follows. Our main result is stated as follows.

\begin{theorem} There exists small positive constants $\eps,\gamma>0$ such that given an instance $X\subseteq \R^M$ of $N$ points, $\mathcal{C}\subseteq \R^M$ and an integer $k$, it is $\mathsf{NP}$-hard to distinguish whether the discrete $k$-means has cost at most $(d-1)N$ or any $(1+\gamma)k$-means clustering solution has cost at least $(d-1)N\left[1+\frac{2}{d(d-1){{2^d}^{\beta}}}\right]$. \end{theorem}

Therefore, discrete $k$-means is hard to approximate within a factor of $\left[1+\frac{2}{d(d-1){{2^d}^{\beta}}}\right]$, even when we are allowed to use $(1+\gamma)$ times more centers. The bicriteria hardness of discrete $k$-median problem can be proved similarly.

